Development and Verification of a Flight Stack for a High-Altitude Glider in Ada/SPARK 2014

SPARK 2014 is a modern programming language and a new state-of-the-art tool set for development and verification of high-integrity software. In this paper, we explore the capabilities and limitations of its latest version in the context of building a flight stack for a high-altitude unmanned glider. Towards that, we deliberately applied static analysis early and continuously during implementation, to give verification the possibility to steer the software design. In this process we have identified several limitations and pitfalls of software design and verification in SPARK, for which we give workarounds and protective actions to avoid them. Finally, we give design recommendations that have proven effective for verification, and summarize our experiences with this new language.

==> section-rules.tex <==

\section{A Rule Set for Co-Verification}
These rules ensure: 
\begin{itemize}
\item consistency of the prover result it itself
\item no masking of errors occurs
\item ...
\end{itemize}

\subsection{Consistency Rules}

\begin{itemize}
\item \textbf{rule:} code must not be modified to reach AoRTE based on proof attempts that ran into timeout/memout/stepout (see \texttt{Lim} function). Instead, increase steps/time or apply \texttt{Assert\_and\_cut};
\item \textbf{rule:} necessary: contracts must be proven AoRTE,
  otherwise we get false negatives \textbf{upstream}, which is
  unintuitive and likely to cause big problems. sufficient: body must
  also be AoRTE, otherwise RTE in post can be masked.


\item \textbf{rule:} sufficient: we can only rely on the proofs in a
  subprogram, if all its dependencies are met, which in particular
  includes the bodies and postcondition of all callees.
\item \textbf{false negatives} skew the picture and can hide dangerous run-time exceptions
  \begin{itemize}
  \item cause exceptions that are not anticipated
  \item \textbf{rule:} we can only trust any verified CV within a subprogram if the subprogram itself is completely free of RTE and has a verified pre- and Postcondition
  \item if Post is not verified and exceptions are off, then errors propagate wildly (obviously), which should be avoided at all cost. 
  \item \textbf{rule:} assuming exceptions are not turned off before \textbf{all} VCs are verified: in contrast to Model Checking with CBMC, a subprogram with non-verified VCs cannot generate false negatives in other subprograms (exception to this rule: inlining in the analysis). Therefore, deductive verification - or more general, assume-guarantee reasoning at pre- and post-condition of functions - limits propagation of error conditions and gives a more certain picture on ``verification success''.
  \item \textbf{false positives} (developer knows that the prover has insufficient knowledge) due to insufficient solver knowledge can also hide dangerous run-time exceptions (GPS failure)
    \begin{itemize}
    \item \textbf{rule:} suppressing false positives should be avoided. If necessary, then include an \texttt{Assert\_And\_Cut} after the suppressed statement, to reset solver knowledge on the specific item that cause the check to fail. E.g., when length check fails, then \texttt{Assert\_And\_Cut(arr'Length >= 0)}, to remove all possibly incorrect assumptions on the array length and thereby unhide downstream false negatives.
    \end{itemize}
  \end{itemize}
  \item RTS requires careful configuration and cannot be abstracted completely
  \item E.g., if architecture details are incorrect (S'Denorm) then
    some runtime checks may fail unexpectedly because target does not
    behave as claimed
  \item can refute the soundness of analysis

\end{itemize}



%%% Local Variables: ***
%%% mode:latex ***
%%% TeX-master: "paper.tex"  ***
%%% End: ***

==> section-workflow.tex <==
\section{Daily Development \& Verification Workflow}
\label{sec:verification}
\todo{cross-verification: how to}
We have developed and verified the onboard software of the glider in parallel for two reasons: 
\begin{enumerate}
\item To let verification needs steer design refinement and
  implementation decisions, and 
\item to get an early grasp on verification efforts, and avoid that
  verification would be done in the last minute, possibly posing
  difficulties or even exposing an unverifiable implementation.
\end{enumerate}
We used two mechanisms were to realize such a co-verification
approach. First, the developers were also responsible for
verification. Besides taking and realizing implementation choices,
their job was to ensure that a minimal set of annotations were
provided (as required per the SPARK language, e.g., state
abstraction), such that static analysis can process their packages.
They also had the option to run the static analysis locally on their
machines. However, analyzing the complete flight stack with sufficient
depth would have taken too long, so local runs were usually limited to
the subprogram they were working on, and with short timeouts
only. This helped them to identify simple defects early, such as
out-of-bounds access to arrays.

Second, we had set-up a Jenkins server to perform nightly analysis
runs on the whole flight stack, with a longer
timeout. One such run could take up to one hour on an octa-core machine
(\SI{2.7}{GHz} Intel Xeon E5-2680 processor with \SI{16}{GB} RAM); note that the
analysis makes full use of all cores. Every time the server had
finished analyzing the project, artifacts summarizing the verification
were emailed to the developers, most importantly:
\begin{inparaenum}
\item the log files of the analysis, showing detailed outputs such as
  warnings, errors and counterexamples and
\item a tabular verification summary.% as shown in Tab.~\ref{tab:cov}. 
\end{inparaenum}
%
% The verification summary table is showing all packages, sorted
% descendingly first by \emph{coverage}, then by \emph{success}. We
% denote as \emph{coverage}, the percentage of SPARK code relative to
% all code in a package. A coverage of 100\% can only be reached if all
% entities in the package body are in SPARK, which includes instances of
% generics, and if all callees of other packages have at least a SPARK
% specification. We denote as \emph{success} the percentage of
% successfully verified properties over all properties.  
%
~These artifacts were used every morning to decide where development
and verification efforts should continue. The goal was reach foll coverage and maximum verification success in the flight-critical packages.

% \bgroup
% \scriptsize
% \setlength\tabcolsep{.45em}
% \begin{table}[btp]
% \begin{minipage}{\linewidth}
%   \centering
%   \caption{Example of a nightly verification summary.}
%     \small
%   \begin{tabular}{lrrrrrr}
%     \toprule
%     Unit & \#entities & \#skip & coverage \% & \#properties & \#proven & success \%\\
%     \midrule
% px4io.protocol & 1 & 0 &  100 & 54 & 54 & 100.0\\
% ublox8.driver & 17 & 0 &  100 & 205 & 202 & 98.5\\
% units.navigation & 16 & 0 &  100 & 109 & 93 & 85.4\\
% \vdots&\vdots&\vdots&\vdots&\vdots&\vdots\\
% mystrings & 8 & 1 & 88 & 18 & 18 & 100.0\\
% controller & 25 & 3 &  88 & 139 & 119 & 85.6\\
% estimator & 25 & 3 &  88 & 175 & 148 & 84.6\\
% \vdots&\vdots&\vdots&\vdots&\vdots&\vdots\\
% fat\_filesystem.directories & 9 & 9 &  0 & 0 & 0 & --\\
%     \bottomrule
%   \end{tabular}\label{tab:cov}
%   \textbf{Totals:} entities: 1062, success: 89.9\%, proven: 2274, coverage:  32.5\%, props: 2531, units: 106
% \end{minipage}
% \end{table}
% \egroup

\textbf{Failing checks} have been investigated by placing additional
assertions to probe the knowledge of the solver, and with that
identify the underlying reason and propose a rewrite that could be
verified. If a failing property depended on a fact that was not
visible to the solver (e.g., the implicitly known length of integer
images), then \texttt{pragma Assume} has been used to provide
knowledge to the analyzer, or, alternatively, a wrapper function was
introduced with a post-condition stating the new fact. If a result was
identified as False Positive, then we applied \texttt{pragma Annotate}
to suppress the warning. Finally, for unclear cases we placed an
\texttt{pragma Assert}, which has the same effect as \texttt{pragma
  Assume}, but leaves a failing VC marking such cases, and potentially
produces a run-time exception which then can be used to understand
such cases.

%%% Local Variables: ***
%%% mode:latex ***
%%% TeX-master: "paper.tex"  ***
%%% End: ***
